Identifiable Causal Representation Learning: Unsupervised, Multi-View, and Multi-Environment

Causal models provide rich descriptions of complex systems as sets of mechanisms by which each variable is influenced by its direct causes. They support reasoning about manipulating parts of the system and thus hold promise for addressing some of the open challenges of artificial intelligence (AI), such as planning, transferring knowledge in changing environments, or robustness to distribution shifts. However, a key obstacle to more widespread use of causal models in AI is the requirement that the relevant variables be specified a priori, which is typically not the case for the high-dimensional, unstructured data processed by modern AI systems. At the same time, machine learning (ML) has proven quite successful at automatically extracting useful and compact representations of such complex data. Causal representation learning (CRL) aims to combine the core strengths of ML and causality by learning representations in the form of latent variables endowed with causal model semantics. In this thesis, we study and present new results for different CRL settings. A central theme is the question of identifiability: Given infinite data, when are representations satisfying the same learning objective guaranteed to be equivalent? This is an important prerequisite for CRL, as it formally characterises if and when a learning task is, at least in principle, feasible. Since learning causal models, even without a representation learning component, is notoriously difficult, we require additional assumptions on the model class or rich data beyond the classical i.i.d. setting. By partially characterising identifiability for different settings, this thesis investigates what is possible for CRL without direct supervision, and thus contributes to its theoretical foundations. Ideally, the developed insights can help inform data collection practices or inspire the design of new practical estimation methods.

==> Preamble/preamble.tex <==
%
%
%

%
%
%
\ifsetCustomMargin
  \RequirePackage[left=37mm,right=30mm,top=35mm,bottom=30mm]{geometry}
  \setFancyHdr %
\fi

%
%
%
\raggedbottom
%
\usepackage[shortlabels]{enumitem}
\setlist[enumerate,itemize,description]{topsep=0em}

%
%

%

\ifsetCustomFont
  %
  %
  %

  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
\fi

%
%

%

%


%

%
%

\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.} %


%

%
%

%
%
%
%

%
%
%
%
\usepackage{subcaption}

%
\usepackage{booktabs} %
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{multicol}
%
\usepackage{tabularx}


%
\usepackage{siunitx} %


%

%
%

%
 \onehalfspacing
%


%

%
\clubpenalty=500
\widowpenalty=500

\usepackage[perpage]{footmisc} %


%
%

%

%
\ifuseCustomBib
   %

%

%
%
%

\fi

%
%


%
%
%

%

\renewcommand{\contentsname}{Table of Contents}
\renewcommand{\listfigurename}{List of Figures}
\renewcommand{\listtablename}{List of Tables}


%

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}


%

%


\usepackage[intoc]{nomencl}
\makenomenclature
\usepackage{xstring}
%
%
%
%

\newcommand{\nomenclheader}[1]{%
	\item[\hspace*{-\itemindent}\normalfont\bfseries#1]}
\renewcommand\nomgroup[1]{%
	\IfStrEqCase{#1}{%
		{A}{\nomenclheader{Random Variables}}
		{Z}{\nomenclheader{Acronyms and Abbreviations}}
		{C}{\nomenclheader{Scalars, Vectors, Matrices}}
		{S}{\nomenclheader{Spaces}}
		{E}{\nomenclheader{Functions}}
  		{F}{\nomenclheader{Derivatives}}
		{D}{\nomenclheader{Probabilities}}
		{G}{\nomenclheader{Graphs}}
	}%
}
\renewcommand\nomname{Notation and Terminology}




%

%

%
%

%

%
%

%
%
%

%
%

%
%

%
%
%


%
%

%
%
%
%
%
%
%

%

%
%
\usepackage{enumitem}


%
%
%


\linepenalty=50

\usepackage{parskip}
\usepackage[dvipsnames]{xcolor}         %
\definecolor{lightgray}{RGB}{196,196,196}
\definecolor{lightblue}{RGB}{34,94,196}
\definecolor{darkred}{RGB}{133,46,43}
\definecolor{darkgreen}{RGB}{0,163,0}
%
\definecolor{blue_cblind}{HTML}{1A85FF}
\definecolor{red_cblind}{HTML}{D41159}
\usepackage{lipsum}
\usepackage{nicefrac}
\usepackage{easyReview}
\usepackage{quoting}
\usepackage{wrapfig}
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows, shadows, bayesnet}
\usepackage{tcolorbox}
\usepackage{amsthm,thmtools,thm-restate}
\usepackage{cleveref}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{mathtools}
\RequirePackage{amsthm}
\usepackage{nccmath}
\usepackage{overpic}
\usepackage{titlesec}
\usepackage{centernot}
\usepackage[12pt]{moresize}
\usepackage{gensymb}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

  
%
%
%
\crefname{figure}{Fig.}{Figs.}
\crefname{definition}{Defn.}{Defns.}
\crefname{corollary}{Cor.}{Cors.}
\crefname{proposition}{Prop.}{Props.}
\crefname{theorem}{Thm.}{Thms.}
\crefname{remark}{Remark}{Remarks}
\crefname{principle}{Principle}{Principles}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{claim}{Claim}{Claims}
\crefname{table}{Tab.}{Tabs.}
\crefname{chapter}{Chapter}{Chapters}
\crefname{part}{Part}{Parts}
\crefname{section}{\S}{\S\S}
\crefname{subsection}{\S}{\S\S}
\crefname{subsubsection}{\S}{\S\S}
\crefname{assumption}{Asm.}{Asms.}
\crefname{appendix}{Appx.}{Appx.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{example}{Example}{Examples}

\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{mathtools}
\ifx\proof\undefined 
\RequirePackage{amsthm}
\fi
\RequirePackage{bm} 
\RequirePackage{url}


%
\newcommand{\wbt}{{\tilde{{\bm{\wb}}}}}
\newcommand{\sbt}{{\tilde{{\bm{\sb}}}}}
\newcommand{\fbt}{{\tilde{{\bm{\fb}}}}}
\newcommand{\Wbt}{{\tilde{{\bm{\Wb}}}}}
\newcommand{\IMA}{\textsc{ima}}
\newcommand{\BSS}{\textsc{bss}}
\newcommand{\IGCI}{\textsc{igci}}
\newcommand{\LIN}{\textsc{lin}}


%


%
%
\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\cb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mbb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{{\bm{v}}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}
\renewcommand{\sb}{\mathbf{s}}
\newcommand{\nb}{\mathbf{n}}
%
\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}


%
%
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

%
%
\newcommand{\CC}{\mathbb{C}} %
\newcommand{\DD}{\mathbb{D}} %
\newcommand{\EE}{\mathbb{E}} %
\newcommand{\VV}{\mathbb{V}} %
\newcommand{\II}{\mathbb{I}} %
\newcommand{\KK}{\mathbb{K}} %
\newcommand{\LL}{\mathbb{L}} %
\newcommand{\MM}{\mathbb{M}} %
\newcommand{\NN}{\mathbb{N}} %
\newcommand{\PP}{\mathbb{P}} %
\newcommand{\QQ}{\mathbb{Q}} %
\newcommand{\RR}{\mathbb{R}} %
\newcommand{\XX}{\mathbb{X}} %
\newcommand{\YY}{\mathbb{Y}} %
\newcommand{\ZZ}{\mathbb{Z}} %
\newcommand{\Cbb}{\mathbb{C}} %
\newcommand{\Dbb}{\mathbb{D}} %
\newcommand{\Ebb}{\mathbb{E}} %
\newcommand{\Vbb}{\mathbb{V}} %
\newcommand{\Ibb}{\mathbb{I}} %
\newcommand{\Kbb}{\mathbb{K}} %
\newcommand{\Lbb}{\mathbb{L}} %
\newcommand{\Mbb}{\mathbb{M}} %
\newcommand{\Nbb}{\mathbb{N}} %
\newcommand{\Pbb}{\mathbb{P}} %
\newcommand{\Qbb}{\mathbb{Q}} %
\newcommand{\Rbb}{\mathbb{R}} %
\newcommand{\Xbb}{\mathbb{X}} %
\newcommand{\Ybb}{\mathbb{Y}} %
\newcommand{\Zbb}{\mathbb{Z}} %


%
\newcommand{\indfone}{\bm{1}}
\newcommand{\1}{\bm{1}}
\newcommand{\Covar}{\mathbb{C} \mathrm{ov} } %

%
%
\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\subto}{\mathop{\mathrm{subject}\;\mathrm{to}}}
%
\newcommand*{\minip}{\mathop{\mathrm{minimize}\;\;}}
\newcommand*{\maxip}{\mathop{\mathrm{maximize}\;\;}}
\newcommand*{\subtop}{\mathop{\mathrm{subject}\;\mathrm{to}\;\;}}
\newcommand*{\argmin}{\mathop{\mathrm{arg\,min}}}
\newcommand*{\argmax}{\mathop{\mathrm{arg\,max}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\suchthat}{\mathrm{s.t.}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\DeclareMathOperator*{\Var}{{\rm Var}}
\DeclareMathOperator*{\Corr}{Corr}
\DeclareMathOperator*{\Cov}{Cov}
\DeclareMathOperator*{\ind}{1{\hskip -2.5 pt}\hbox{I}}  %
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}  

\newcommand*{\zero}{{\bf 0}}
\newcommand*{\one}{{\bf 1}}

\newcommand*{\Risk}{{\rm Risk}}
\newcommand*{\Bias}{{\rm Bias}}

\newcommand{\pen}{{\rm pen}}
\newcommand{\diag}{{\rm diag}}
\newcommand{\diam}{{\bf{\rm diam}}}
\newcommand{\spann}{{\bf{\rm span}}}
\newcommand{\nulll}{{\bf{\rm null}}}
\newcommand{\vol}{{\bf{\rm vol}}}

%
\newcommand{\rank}{{\bf{\rm rank}}}
\newcommand{\dimension}{{\bf{\rm dim}}}

%
\newcommand{\epi}{{\bf{\rm epi}}\;}
\newcommand{\hypo}{{\bf{\rm hypo}}\;}

%
%
\newcommand{\dom}{{\bf{\rm dom}}\;} %
\newcommand{\interior}{{\bf{\rm int}}\;} %

%
\newcommand{\bigO}{\tilde{O}}
\newcommand{\bigOtilde}{\tilde{\mathcal{O}}}
\newcommand{\littleO}{\mathcal{o}}
\newcommand{\bigOmega}{\mathcal{\Omega}}
\newcommand{\littleOmega}{\mathcal{\omega}}

%
\newcommand{\Bern}{{\bf{\rm Bern}}\,} %
\newcommand{\Categ}{{\bf{\rm Categ}}\,} %
\newcommand{\Mult}{{\bf{\rm Mult}}\,} %
\newcommand{\Dir}{{\bf{\rm Dir}}\,} %

%
\newcommand{\differentiate}[2]{ \frac{ \ud #2}{\ud #1} }
\newcommand{\differentiateat}[3]{ \frac{ \ud #2}{\ud #1}  \Big|_{#1=#3} }
\newcommand{\partialfrac}[2]{ \frac{ \partial #2}{\partial #1} }
\newcommand{\partialfracat}[3]{ \frac{ \partial #2}{\partial #1} \Big|_{#1=#3} }
\newcommand{\partialfracorder}[3]{ \frac{ \partial^{#3} #2}{\partial^{#3} #1} }
\newcommand{\partialfracatorder}[4]{ \frac{ \partial^{#3} #2}
	{\partial^{#3} #1} \Big|_{#1=#4} }

%
\newcommand{\defeq}{\stackrel{\Delta}{=}}

%
\newcommand{\indistribution}{\xrightarrow[]{\Dcal}}
\newcommand{\inprobability}{\xrightarrow[]{\Pcal}}

\def\iid{{i.i.d }}
\newcommand{\iidsim}{\stackrel{{iid}}{\sim}}
\def\bks{\backslash}

%
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

%
\renewcommand{\emptyset}{\varnothing}

%
%
\newcommand*{\alphab}{\bm{\alpha}}
\newcommand*{\betab}{\bm{\beta}}
\newcommand*{\Sigmab}{\bm{\Sigma}}
\newcommand*{\Omegab}{\bm{\Omega}}
\newcommand*{\omegab}{{\bm{\omega}}}
\newcommand*{\Gammab}{\bm{\Gamma}}
\newcommand*{\Psib}{\bm{\Psi}}
\newcommand*{\Thetab}{\bm{\Theta}}
\newcommand*{\thetab}{\bm{\theta}}
\newcommand*{\taub}{\bm{\tau}}
\newcommand*{\epsilonb}{\bm{\epsilon}}
\newcommand*{\etab}{\bm{\eta}}
\newcommand*{\xib}{\bm{\xi}}
\newcommand*{\gammab}{\bm{\gamma}}
\newcommand*{\deltab}{\bm{\delta}}
\newcommand*{\Deltab}{\bm{\Delta}}
\newcommand*{\mub}{\bm{\mu}}
\newcommand*{\rhobb}{\bm{\rho}}
\newcommand*{\Phib}{\bm{\Phi}}
\newcommand*{\phib}{\bm{\phi}}

%


%
\newcommand{\orlnorm}[2]{||#1||_{\Psi_{#2}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\smallnorm}[1]{\lVert#1\rVert}
\newcommand{\bignorm}[1]{\bigg|\bigg|#1\bigg|\bigg|}
\newcommand{\opnorm}[2]{| \! | \! | #1 | \! | \! |_{{#2}}}

%
\newcommand{\dotp}[2]{\langle{#1},{#2}\rangle}

%
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}


%
\newcommand{\mcomment}[1]{\marginpar{\tiny{#1}}}
\newcommand{\fcomment}[1]{\footnote{\tiny{#1}}}


%
%
%

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  %
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi
%
\ifx\proofsketch\undefined
\newenvironment{proofsketch}{\par\noindent{\bf Proof Sketch\ }}{\hfill\BlackBox\\[2mm]}
\fi

\theoremstyle{plain} %
\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{chapter}
\fi
\ifx\property\undefined
\newtheorem{property}{Property}
\fi
\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi
\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi
\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi
\ifx\assum\undefined
\newtheorem{principle}[theorem]{Principle}
\fi

\theoremstyle{definition} %
\ifx\definition\undefined
\newtheorem{definition}[theorem]{Definition}
\fi
\ifx\assum\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

\ifx\example\undefined
\newtheorem{example}[theorem]{Example}
\fi
\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi
\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi
\ifx\fact\undefined
\newtheorem{fact}[theorem]{Fact}
\fi
\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi
\ifx\assum\undefined
\newtheorem{observation}[theorem]{Observation}
\fi

\theoremstyle{remark} %
\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi




\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\nindep}{\not\independent}


\delimitershortfall-1sp
\newcommand\abs[1]{\left|#1\right|}
\newcommand{\dbtilde}[1]{\tilde{\raisebox{0pt}[0.85\height]{$\tilde{#1}$}}}
\renewcommand*\d{\mathop{}\!\mathrm{d}}

%
%
%


%
%
%
%


%
%
\newcommand{\horizontalline}{\noindent\rule[0.5ex]{\linewidth}{1pt}}
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}} 
\newcommand{\Hrule}{\rule{\linewidth}{0.3mm}}
\newcommand{\HRuleN}{\HRule\\} 
\newcommand{\HruleN}{\Hrule\\}
\newcommand{\superscript}[1]{{\scriptsize \ensuremath{^{\textrm{#1}}}}}
\newcommand{\supindex}[2]{#1^{(#2)}}
\newcommand{\xii}[1]{\supindex{\xb}{#1}}
\newcommand{\yii}[1]{\supindex{y}{#1}}
\newcommand{\zii}[1]{\supindex{\zb}{#1}}
\newcommand{\Xii}[1]{\supindex{\Xb}{#1}}
\newcommand{\Wii}[1]{\supindex{\Wb}{#1}}
\newcommand{\Yii}[1]{\supindex{Y}{#1}}
\newcommand{\Zii}[1]{\supindex{Z}{#1}}

\newcommand{\mut}[2]{\mu_{#1}({#2})}
\newcommand{\sigmat}[2]{\sigma_{#1}({#2})}
\newcommand{\tmut}[2]{\tilde{\mu}_{#1}({#2})}
\newcommand{\tyb}{\tilde{\yb}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tO}{\tilde{O}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\tz}{\tilde{\zb}}
\newcommand{\tT}{\tilde{T}}
\newcommand{\tx}{\tilde{\xb}}
\newcommand{\sigb}{\mathbf{\Sigma}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\txii}[1]{\supindex{\tx}{#1}}

%
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


%
\newcommand{\xbm}{{\bm{x}}}
\newcommand{\sbm}{{\bm{s}}}
\newcommand{\ybm}{{\bm{y}}}
\newcommand{\zbm}{{\bm{z}}}
\newcommand{\vbm}{{\bm{v}}}
\newcommand{\Xbm}{{\bm{X}}}
\newcommand{\Ybm}{{\bm{Y}}}
\newcommand{\Zbm}{{\bm{Z}}}
\newcommand{\Vbm}{{\bm{V}}}
\newcommand{\Xset}{{\set{X}}}
\newcommand{\Yset}{{\set{Y}}}
\newcommand{\Zset}{{\set{Z}}}
\newcommand{\Vset}{{\set{V}}}

\def\-{\raisebox{.75pt}{-}}
\newcommand{\shortminus}{\scalebox{0.75}[1.0]{\( - \)}}
\newcommand{\thetagen}{{\bm{\theta}^{}_g}}
\newcommand{\thetadopt}{{\bm{\theta}^*_d}}
\newcommand{\thetagopt}{{\bm{\theta}^*_g}}
\newcommand{\thetad}{{\bm{\theta}_d}}
\newcommand{\thetade}{{\bm{\theta}_d^e}}
\newcommand{\thetadd}{{\bm{\theta}_d^d}}
\newcommand{\supp}{{\mathrm{supp}}}
\newcommand{\vj}{{\bm{v}_j}}
\newcommand{\vjs}{{\{\bm{v}_j\}_{j=1}^J}}
\newcommand{\allparams}{{(\bm{\theta}_g, \bm{\theta}_d, \mathbf{V})}}
\newcommand{\allparamsours}{{(\bm{\theta}_g, \set{V})}}
\newcommand{\yvbm}{{\bm{yv}}}
\newcommand{\vybm}{{\bm{vy}}}
\newcommand{\vxbm}{{\bm{vx}}}
\newcommand{\xvbm}{{\bm{xv}}}
\newcommand{\xybm}{{\bm{xy}}}
\newcommand{\yxbm}{{\bm{yx}}}
\newcommand{\thetabm}{{\bm{\theta}}}
\newcommand{\omegabm}{{\bm{\omega}}}



\newcommand*{\tran}{^{\mkern-1.5mu\mathsf{T}}}
%
\newcommand{\pa}{\mathrm{pa}}
\newcommand{\nd}{\mathrm{nd}}
\newcommand{\Pa}{\mathbf{Pa}}
\newcommand{\PA}{\mathbf{Pa}}
\newcommand{\CH}{\mathbf{Ch}} %
\newcommand{\DE}{\mathbf{De}} %
\newcommand{\ND}{\mathbf{NDe}} %
\newcommand{\AN}{\mathbf{An}} %

\newcommand{\Ftt}{\texttt{F}}
\newcommand{\cost}{\mathrm{cost}}
\newcommand{\xF}{\xb^\Ftt}
\newcommand{\uF}{\ub^\Ftt}
\newcommand{\vF}{\vb^\Ftt}
\newcommand{\aF}{a^\Ftt}
\newcommand{\A}{A}
\newcommand{\IW}{\textsc{imf}}
\newcommand{\MINT}{\textsc{cau}}
%
\newcommand{\CE}{\textsc{CE}}
\newcommand{\CEs}{\textsc{CE}s}
\newcommand{\SCM}{\textsc{SCM}}
\newcommand{\SCMs}{\textsc{SCM}s }
\newcommand{\thetaI}{\bm{\theta}_\Ical}
\newcommand{\SVM}{\textsc{svm}}

\newcommand{\x}{\mathbf{x}}
\newcommand{\xCE}{\mathbf{x}^\texttt{CE}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\X}{\mathbf{X}}
%
%
\newcommand{\Id}{\mathbf{I}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\AF}{\mathbb{A}^\texttt{F}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\Hil}{\mathcal{H}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\N}{\mathcal{N}}
\renewcommand{\SS}{\mathbf{S}}
\renewcommand{\ss}{\sigma^2}
\newcommand{\GP}{\mathcal{GP}}
\newcommand{\dist}{\text{dist}}
\newcommand{\costF}{\text{cost}^\texttt{F}}
\newcommand{\U}{\mathbf{U}}
\renewcommand{\u}{\mathbf{u}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\I}{\mathcal{I}}
\renewcommand{\th}{{\bm\theta}}
\newcommand{\muF}{\mu^\texttt{F}}
\newcommand{\ssF}{s^\texttt{F}}
\newcommand{\xSCF}{\mathbf{x}^\texttt{SCF}}
\newcommand{\XSCF}{\mathbf{X}^\texttt{SCF}}
%
%
\newcommand{\SH}{\mathbf{S}}
\newcommand{\MH}{\mathcal{M}}
\newcommand{\Mstar}{\mathcal{M}_\star}
\newcommand{\Sstar}{\mathbf{S}_\star}
\newcommand{\CATEstar}{\textsc{cate}_\star}
\newcommand{\Validstar}{\text{Valid}_\star}
\newcommand{\lin}{\textsc{lin}}
\newcommand{\KR}{\textsc{kr}}
\newcommand{\KLD}[2]{D_{\mathrm{KL}} \left( \left. \left. #1 \right|\right| #2 \right) }

\newcommand{\eps}{\epsilon}
\newcommand{\e}{\bm{\epsilon}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\given}{\vert}
\newcommand{\0}{\mathbf{0}}
\newcommand{\LCB}{\textsc{lcb}}
\newcommand{\fig}{Fig.~}
\newcommand{\cate}{\textsc{cate}}
\newcommand{\cvae}{\textsc{cvae}}
\newcommand{\method}{\textsc{method}}
\newcommand{\gp}{\textsc{gp}}
\newcommand{\gpscm}{\textsc{gp-scm}}
\newcommand{\scm}{\textsc{scm}}
\newcommand{\anm}{\textsc{anm}}
%
%
\newcommand{\enc}{E}
\newcommand{\dec}{D}

\newcommand{\cbt}{\Tilde{\cb}}
\newcommand{\Cbt}{\Tilde{\Cb}}
\newcommand{\Sbt}{\Tilde{\Sb}}
\renewcommand{\st}{\Tilde{s}}
\newcommand{\xbf}{\xb^{\texttt{F}}}
\newcommand{\zbf}{\zb^{\texttt{F}}}
\newcommand{\cbf}{\cb^{\texttt{F}}}
\newcommand{\sbf}{\sb^{\texttt{F}}}
\newcommand{\xbcf}{\xb^{\texttt{CF}}}
\newcommand{\zbcf}{\zb^{\texttt{CF}}}
\newcommand{\cbcf}{\cb^{\texttt{CF}}}
\newcommand{\sbcf}{\sb^{\texttt{CF}}}
\newcommand{\gs}{g^\star}
%
\newcommand{\ph}{\hat{p}}
\newcommand{\zbh}{\hat{\zb}}
\newcommand{\cbh}{\hat{\cb}}
\newcommand{\sbh}{\hat{\sb}}
\newcommand{\fbh}{\hat{\fb}}
\newcommand{\zbth}{\hat{\zbt}}
\newcommand{\cbth}{\hat{\cbt}}
\newcommand{\sbth}{\hat{\sbt}}
\newcommand{\Ac}{{\A^\mathrm{c}}}
%
\newcommand{\te}{{\mathrm{te}}}
\newcommand{\MSE}{\mathrm{MSE}}
\newcommand{\MLP}{\mathrm{MLP}}

\newcommand{\xbt}{\Tilde{\xb}}
\newcommand{\ybt}{\Tilde{\yb}}
\newcommand{\zbt}{\Tilde{\zb}}
\newcommand{\gbt}{\Tilde{\gb}}
\newcommand{\Xbt}{\Tilde{\Xb}}
\newcommand{\Zbt}{\Tilde{\Zb}}
\newcommand{\fbinv}{\fb^{-1}}
\newcommand{\hbinv}{\hb^{-1}}
\newcommand{\gbinv}{\gb^{-1}}

\newcommand{\diff}{\,\mathrm{d}}
\newtcolorbox{selfcitebox}{
 colback=Blue!3,
  colframe=Blue,
 boxsep=0em,
	%
	width=\textwidth,
	sharpish corners,
	top=1.5mm, %
	bottom=1.5mm,
	left=1.5mm,
	right=1.5mm
}

\newcommand{\leftkl}{D_{KL}^{\text{left}}}
\newcommand{\sib}{\boldsymbol{\sigma}}
